Explainability and Robustness of Deep Visual Classification Models

In the computer vision community, Convolutional Neural Networks (CNNs), first proposed in the 1980's, have become the standard visual classification model. Recently, as alternatives to CNNs, Capsule Networks (CapsNets) and Vision Transformers (ViTs) have been proposed. CapsNets, which were inspired by the information processing of the human brain, are considered to have more inductive bias than CNNs, whereas ViTs are considered to have less inductive bias than CNNs. All three classification models have received great attention since they can serve as backbones for various downstream tasks. However, these models are far from being perfect. As pointed out by the community, there are two weaknesses in standard Deep Neural Networks (DNNs). One of the limitations of DNNs is the lack of explainability. Even though they can achieve or surpass human expert performance in the image classification task, the DNN-based decisions are difficult to understand. In many real-world applications, however, individual decisions need to be explained. The other limitation of DNNs is adversarial vulnerability. Concretely, the small and imperceptible perturbations of inputs can mislead DNNs. The vulnerability of deep neural networks poses challenges to current visual classification models. The potential threats thereof can lead to unacceptable consequences. Besides, studying model adversarial vulnerability can lead to a better understanding of the underlying models. Our research aims to address the two limitations of DNNs. Specifically, we focus on deep visual classification models, especially the core building parts of each classification model, e.g. dynamic routing in CapsNets and self-attention module in ViTs.

==> conclusion.tex <==
\chapter{Conclusion}

In this dissertation, we have studied the explainability and robustness of deep visual classification models. Especially, we focus on the popular deep visual neural networks, namely, Convolutional Neural Networks (CNNs), Capsule Networks (CapsNets), and Vision Transformers (ViTs). From the perspective of explainability, we propose an explanation tool for CNNs and interpretable CapsNets and provide an understanding of ViT-based classifications. Besides, by studying the core building component of each component, e.g., dynamic routing in CapsNets and self-attention in ViTs, we reveal the weakness of their predictions when natural and adversarial perturbations are injected into input images. The contribution of this thesis will facilitate the application of existing popular deep visual classification models and inspires the development of more intelligent classifiers in the future.


In Chapter 2, we first evaluate the explanations generated by LRP and find that the generated explanations are not class-discriminative. To improve discriminativeness of the generated explanations, we propose the Contrastive Layer-wise Relevance Propagation (CLRP). Both qualitative and quantitative evaluations confirm that the CLRP is better than the LRP. As an explanation tool, our CLRP is able to generate class-discriminative, pixel-wise explanations for the individual CNN-based classification decisions.


In Chapter 3, we propose an interpretable Graph Capsule Networks (GraCapsNet). The built-in explanations for individual classifications of GraCapsNets can be created in an effective and efficient way. Surprisingly, our model also demonstrates some unexpected benefits, even though it replaces the fundamental part of CapsNets. Our GraCapsNets achieve better classification performance with fewer parameters and better adversarial robustness when compared to CapsNets. Besides, GraCapsNets
still keep other advantages of CapsNets, namely, disentangled
representations and affine transformation robustness. When applied to classify images, our GraCapsNet is able to offer classification explanations in an effective and efficient way.


In Chapters 4 and 5, We first analyze the robustness of CapsNets to input affine transformation and attribute their robustness to CapsNet architecture instead of dynamic routing. Based on our exploration of the
limitation of the CapsNet architecture, we propose AffCapsNets, which improves affine transformation robustness significantly using fewer parameters. Furthermore, we summarize 5 major differences between CapsNets and ConvNets and study 3 properties of CapsNets. We show that dynamic routing is harmful to CapsNets in terms of transformation robustness and semantic representations. In each presented task, a simple ConvNet can be built to outperform the CapsNet significantly. Overall, we conclude that \textit{Dynamic Routing Capsule Network is Not More Robust than Primary Convolutional Neural Networks.}   


In Chapter 6, we focus on the adversarial robustness of CapsNets. By revealing how it is affected by adversarial examples, our investigation reveals that adversarial examples can mislead CapsNets by manipulating the votes. We propose an effective and efficient Vote-Attack to attack CapsNets. The Vote-Attack is more effective and efficient than the standard Caps-Attack in both standard training and adversarial training settings. The adversarial robustness of CapsNets can be reduced to a similar level to the counterpart CNNs under our proposed Vote Attack.


In Chapter 7, based on the architectural traits of Vision Transformers, we study the following question interesting: How does ViT perform when individual input image patches are perturbed with natural corruptions or adversarial perturbations, compared to CNNs? Based on a fair comparison, we find that ViT is more robust to natural patch corruption than ResNet,
whereas it is more vulnerable to adversarial patch perturbation. We conduct extensive analysis to understand our observations. Specifically, we reveal that the self-attention mechanism can effectively ignore natural corrupted patches to maintain a correct prediction but be easily fooled to focus on adversarial patches to make a mistake. Inspired by our analysis, we show attention smoothing can improve the robustness of ViT against adversarial patches since smoothed attention does not focus on a single patch. This chapter shows that self-attention boost the robustness to natural patch perturbations, but reduce the robustness to adversarial patch.


We argue that the adversarial vulnerability and the lack of explainability of deep visual classification models can be attributed to the difference between the current deep visual neural network-based classification and human visual recognition. The advanced modules of existing deep vision classification models, i.e., skip connections, dynamic routing, and self-attention, do not necessarily make image classification more aligned with human perception. In this dissertation, we develop tools to make the existing deep visual classifications more explainable and robust and reveal the large gap between the existing deep visual classifications and human-aligned object recognition. We believe that this dissertation will contribute to the application of existing popular deep visual classification models and inspire the development of more human-aligned classification models.


Different from the image classification task, it is often multi-goal oriented for our human perception to recognize objects. For example, during object recognition, we often easily locate objects, segment objects from the cluttered background, and recall the relationship of the object with other concepts. 


In future work, we will study the robustness of visual structured models, e.g., object detection, semantic segmentation, and scene graph generation. Furthermore, we will explore integrating external knowledge to improve the robustness of vision systems, e.g., designing new architectures to leverage text knowledge for improving robustness. Besides the explainability and the robustness, we will also explore the efficiency of the visual systems to facilitate their applications. Especially, we are interested in improving efficiency from the perspective of cognitive perception.


Overall, my research goal is to build explainable, robust, and efficient visual systems. With my research, I am dedicated to making AI more intelligent and safer.
